Accountable authentication with privacy protection: The Larch system for universal login

Credential compromise is hard to detect and hard to mitigate. To address this problem, we present larch, an accountable authentication framework with strong security and privacy properties. Larch protects user privacy while ensuring that the larch log server correctly records every authentication. Specifically, an attacker who compromises a user's device cannot authenticate without creating evidence in the log, and the log cannot learn which web service (relying party) the user is authenticating to. To enable fast adoption, larch is backwards-compatible with relying parties that support FIDO2, TOTP, and password-based login. Furthermore, larch does not degrade the security and privacy a user already expects: the log server cannot authenticate on behalf of a user, and larch does not allow relying parties to link a user across accounts. We implement larch for FIDO2, TOTP, and password-based login. Given a client with four cores and a log server with eight cores, an authentication with larch takes 150ms for FIDO2, 91ms for TOTP, and 74ms for passwords (excluding preprocessing, which takes 1.23s for TOTP).

==> figs/ecdsa-proto.tex <==
\begin{framed}
    {\small
    The ECDSA signature scheme for message space $\calM$ uses a group
    $\G$ of prime order $q$
    and is parameterized by a hash function $\Hash: \calM \to \Z_q$ and
    a conversion function $f: \G \to \Z_q$.
    An ECDSA keypair is a pair $(y, g^y) \in \Z_q \times \G$ for
    $y \getsr \Z_q$. 
    We use a secure multiplication protocol $\PiMul$ (\cref{fig:halfmul}
    in \cref{app:secdefs:halfmul})
    and a secure opening protocol $\PiOpen$ that returns the result or $\bot$
    (``output'' step in Figure 1 of SPDZ~\cite{SPDZ12}).

    \medskip
    
    \underline{$\LogKeyGen() \to (\sksiglog, \pksiglog)$:}
            \begin{itemize}
                \item Sample $x \getsr \Z_q$ and output $(x, g^{x})$.
            \end{itemize}
    \smallskip
    \underline{$\PreSign() \to (\presig_0, \presig_1)$:}
            \begin{itemize}
                \item Sample $r \getsr \Z_q^\ast$ and compute $R \gets f(g^{r})$.
                \item Sample $\alpha \getsr \Z_q$ and compute
                    $\hat{r} \gets \alpha \cdot r^{-1}$.
                \item Split $r^{-1}$ into secret shares $r_0, r_1$;
                    $\hat{r}$ into $\hat{r_0}, \hat{r_1}$;
                    $\alpha$ into $\alpha_0, \alpha_1$;
                \item Output $(R, r_0, \hat{r_0}, \alpha_0)$,
                    $(R, r_1, \hat{r_1}, \alpha_1)$.
            \end{itemize}
    \smallskip
    \underline{$\ClientKeyGen(\pksiglog) \to (\sksigclient, \pk)$:}
            \begin{itemize}
                \item Sample $y \getsr \Z_q$.
                \item Output $(y, \pksiglog \cdot g^{y})$.
            \end{itemize}

    \smallskip
    
    \underline{$\Pi_\Sign$:}

    \smallskip
    
    We refer to the log as party $0$ and the client as party $1$.
    The input of party $i \in \zo$ is $(m, \sk_i, \presig_i)$,
    and the output is a signature $\sigma$ on $m$ or $\bot$.
  
    \smallskip

        For each party $i \in \zo$:
        \begin{itemize}
            \item Party $i$ parses $\presig_i$ as $(R, r_i, \hat{r_i}, \alpha_i)$.
            \item Given input $(r_i, \hat{r_i}, \sk_i, \alpha_i)$ for party $i$,
                run $\PiHalfMul$ to compute shares $(x_i, \hat{x_i}, v_i, \hat{v_i})$
                where $\hat{v_i}$ authenticates any intermediate 
                values.
            \item Party $i$ computes $s_i \gets r_i \cdot \Hash(m) + x_i \cdot R $.
            \item Party $i$ computes $\hat{s_i} \gets \hat{r_i} \cdot \Hash(m) + \hat{x_i} \cdot R $.
            \item Parties run $\PiOpen$ with party $i$ input $\alpha_i, s_i, \hat{s_i}, v_i, \hat{v_i}$
                to get $s$ or $\bot$ (if returns $\bot$, output $\bot$).
            \item Output $(R,s)$.
        \end{itemize}
        }
\end{framed}


==> figs/proto.tex <==
\begin{figure}
\begin{framed}
{\small
\begin{tabular*}{\columnwidth}{l l @{\extracolsep{\fill}} r c r}
%\begin{tabular*}{\linewidth}{l @{\extracolsep{\fill}} c c c r}

\textbf{RP} & & \multicolumn{1}{c}{\textbf{Client}} & & \textbf{Log} \\
\hline \\
multicolumn{4}{l}{\underline{$\authenticate(\id, \authid, \stin) \to \stout$}:} \\
\smallskip \\
&& Parse $\stin$ as $(k,r,h)$ &&\\
\figureLeftArrow{$\authid$} &&\\
\figureRightArrow{$\rpid, \chal$} &&\\[12pt]
\smallskip \\
&& $\ct \gets \Enc(k, \rpid)$ && \\
&& $c \gets \Comm(r, k)$ && \\
&& $m \gets H(\chal || \rpid)$ && \\
&&&& \\
&& Generate proof $\pi$ for && \\
&& \quad input $(\ct, c, m)$ and && \\
&& \quad witness $(k, \rpid, \chal, r)$. && \\
%& \quad certifying: && \\
%& $ \quad \bullet~ \ct = \Enc(k, \rpid)$ && \\
%& $ \quad \bullet~ c = \Comm(r,k)$ && \\
%& $ \quad \bullet~ m = H(\chal, \rpid)$ && \\
& \figureRightArrow{$\pi, \id, \ct, m$} \\
&&&& Get $c$ for $\id$ \\
&&&& Verify $\pi$ on \\
&&&& $(\ct, c, m)$ \\
&& \figureBothArrow{Sign $m$, output $\sigma$} \\
%&& \multicolumn{1}{c}{$\sigma$} && \\
\figureLeftArrow{$\sigma$} && \\
\end{tabular*}
}
\end{framed}
\end{figure}
    \emma{move statement being proved to text}

